CRQBench: A Benchmark of Code Reasoning Questions

Large Language Models have demonstrated exceptional proficiency on coding tasks, but it is challenging to precisely evaluate their code reasoning ability. Existing benchmarks are insufficient as they are unrealistic and conflate semantic reasoning ability with performance on software engineering tasks. We introduce CRQBench, a benchmark of 100 C++ code reasoning questions and answers derived from contextualized code review comments. To curate CRQBench, we use an LLM assistant alongside human inspection, reducing manual effort. We conduct an evaluation of GPT-4 on CRQBench and find that it produces correct responses grounded in the given context for 65 of the 100 questions.

==> sections/evaluation.tex <==
\section{Evaluation}
\label{sec:eval}

%\begin{itemize}
 %   \item RQ1: Is our code reasoning classifier effective?
%    \item RQ2: Is our comment to question rephraser effective?
%\end{itemize}

\subsection{Code Reasoning Classification}


\subsection{Comment to Question Rephrasing}


%\begin{comment}
%\begin{table}[h]
%\begin{tabular}{c|cc}
%\toprule
%                & Corp & Github  \\ \hline
%Precision       & .66                       & .63                    \\ 
%Recall          & \todo{?}                        & .63                         \\ 
%F1 Score        & \todo{?}                        & .63                         \\ \bottomrule
%\end{tabular}
%\caption{Comment to Code Reasoning Question Rephrasing Performance.}
%\label{tab:rephraser}
%\end{table}
%\end{comment}


%Our experimental setup is 2400 randomly selected contextualized code review comments. We evaluate our rephrasing as an entire end-to-end process. That is, from query classification to validation, if a final code reasoning question is output, is it considered a correct rephrase? Of the 2400 input comments, 74 rephrased questions were presented to the human for validation. 49 of them were verified as correct rephrasings, giving a precision of .66.  Ultimately, in order to curate a benchmark of 100 samples, a manual curator would need to inspect 500 samples, and manually curate the underlying question and answers for 100. In contrast, a human validator using our approach would only need to inspect 150 rephrased comments and curate answers. This reduces the number of samples needed to inspect as well as eliminating the need for manually rephrasing the comment into a CRQ. 



==> sections/future.tex <==
\section{Conclusion and Future Work}
In summary, we present a benchmark of 100 code reasoning questions, answers, and corresponding code contexts for evaluating a model's ability to reason over semantic properties of code. To curate this benchmark, we use a cooperative LLM and human inspection technique to reduce manual human effort. In terms of future work, the benchmark could be expanded to include samples in languages beyond C++. Furthermore, performance improvements in the cooperative approach, most notably answer curation, could reduce manual effort further while reducing the number of samples needed prior to classification.  


%Additional Languages: This work was done on C++ code reviews. We do not have a grasp on its level of effectiveness and ability to generalize to other languages. 
%Further Benchmark Evaluation: The effectiveness of each design decision in our technique was not evaluated. We only evaluated comment rephrasing end-to-end rather than an evaluation of error at each step. Furthermore, the quality and difficulty of the questions were not evaluated. A distribution of question “difficulty” may be useful. For example, how many samples require interprocedural analysis?

==> sections/prompts.tex <==
\begin{verbatim}

code_reasoning_classifier =
"""You are a senior, expert C/C++ programmer with a lot of experience analyzing C/C++ code.
Given a C/C++ line comment:

{ROOT_COMMENT}

associated with this line of code:

```
{CODE_SEGMENT}
```

please determine which of the following categories best classifies that
line comment:

1. unknown: unknown
2. reasoning: a code reasoning question such as requiring control-flow or value propagation
3. explanation: a question asking what the code does
4. structure: request to reorganize or refactor code, such as extracting classes or methods
5. planning: prioritization, planning, or choosing what to work on next
6. style: a code simplicity, style, or readability question including things like renaming symbols
7. format: a comment or question about code formatting

and provide an explanation of why that comment should be in that specific category.
If you are uncertain about the category, respond with "0".

Generate your output in YAML format like this:

Explanation: <why you chose a specific category>
Line comment category: <category>

Response:
```yaml"""

\end{verbatim}

\begin{verbatim}

COMMENT_P1 = "also check if the tf example is empty?"
P1_CLASS = No

// 2 No, 3 Yes examples.

query_type_classifier = """You are an expert software engineer, asked to determine whether or not
a reviewer comment is about substituting code.

Here are some examples.

Example 1:

LINE_COMMENT:
```
{COMMENT_P1}
```

1. {P1_CLASS}

Example 2:

LINE_COMMENT:
```
{COMMENT_P2}
```

1. {P2_CLASS}

Example 3:

LINE_COMMENT:
```
{COMMENT_P3}
```

1. {P3_CLASS}

Example 4:

LINE_COMMENT:
```
{COMMENT_P4}
```

1. {P4_CLASS}

Example 5:

LINE_COMMENT:
```
{COMMENT}
```

1."""

\end{verbatim}

\begin{verbatim}
'''
You are an expert C++ coder and know how to review C++ code at Google, and how to respond to reviewer comments.
In the code below, a reviewer has left a comment marked by LINE_COMMENT.

Code:
```
{CODE_SEGMENT_WITH_COMMENT}
```

The comment is asking to consider the following original code and modified code:
'''

\end{verbatim}

\begin{verbatim}

equiv_edit_generator = '''Can you please rephrase a reviewer LINE_COMMENT that suggests the following code change? The rephrased comment should include program elements. Here are a few examples.

Example 1:

Before:
```
{BEFORE}
```

After:
```
{AFTER}
```

[*] [LINE_COMMENT] {MY_LINE_COMMENT}
Rephrased: {Q_C}

Example 2:

Before:
```
{BEFORE_2}
```

After:
```
{AFTER_2}
```

[*] [LINE_COMMENT] {MY_LINE_COMMENT_2}
Rephrased: {Q_C_2}

Example 3:

Before:
```
{BEFORE_i}
```

After:
```
{AFTER_i}
```

[*] [LINE_COMMENT] {MY_LINE_COMMENT_i}'''


\end{verbatim}


\begin{verbatim}
expression_extractor = ''''
You are an expert C++ coder and know how to review C++ code at Google, and how to respond to reviewer comments.
In the code below, a reviewer has left a comment marked by LINE_COMMENT.

Please answer the following question.
1. Can you please list the relevant program expression?

Here are some examples.

Example 1:

Code:
```
{CODE_SEGMENT_WITH_COMMENT_P1}
```

LINE_COMMENT: {COMMENT_P1}

1. {P1_EXPR}

Example 2:

Code:
```
{CODE_SEGMENT_WITH_COMMENT_P2}
```

LINE_COMMENT: {COMMENT_P2}

1. {P2_EXPR}

Example 3:

Code:
```
{CODE_SEGMENT_WITH_COMMENT}
```

LINE_COMMENT: {COMMENT}

'''
\end{verbatim}

\begin{verbatim}

may_rewrite = ''''
You are an expert C++ coder and know how to review C++ code at Google, and how to respond to reviewer comments.
A reviewer has left a comment marked by LINE_COMMENT.

Can you please rephrase the LINE_COMMENT as a question over program expressions?
The Question should start with the word "Can".

Here are some examples.

Example 1:

Comment:
```
{COMMENT_P1}
```

Program Expression: {P1_EXPR}
Question: {P1_Q_C}

Example 2:

Comment:
```
{COMMENT_P2}
```

Program Expression: {P2_EXPR}
Question: {P2_Q_C}

Example 3:

Comment:
```
{COMMENT}
```

Program Expression: {EXPR}'''

\end{verbatim}


\begin{verbatim}
    
validator = '''
You are an expert C++ coder and know how to review C++ code at Google, and how to respond to reviewer comments.
In the code below, a reviewer has left a comment marked by LINE_COMMENT.

Code:
```
{CODE}
```

Given the LINE_COMMENT, answer the following question with YES or NO:
Does ```{Q_C}``` have the same meaning as the LINE_COMMENT?
'''

\end{verbatim}



Uninteresting Keywords:
test
“nit” 
“follow up”
“log a higher level” 
log a lower level 
 logging
“naming”
“readability”
“TODO”
“Description”
“Comment”
Typo
Clang
Style guide
“Period”
Restructure
Restructuring 
Refactor
Move 
Offline
Space
spacing

Interesting Keywords:
"except", 
"segfault"
" fault"
"precondition"
 "assumption", 
"undefined behavior",
 " ub " 
"null", 
"reach", 
"ever be true",
"ever be false", "
branch taken", 
"branch not taken", 
"deref"
"reference"



